An In-Situ Spatial-Temporal Sequence Detector for Neuromorphic Vision Sensor Empowered by High Density Vertical NAND Storage

Neuromorphic vision sensors require efficient real-time pattern recognition, yet conventional architectures struggle with energy and latency constraints. Here, we present a novel in-situ spatiotemporal sequence detector that leverages vertical NAND storage to achieve massively parallel pattern detection. By encoding each cell with two single-transistor-based multi-level cell (MLC) memory elements, such as ferroelectric field-effect transistors (FeFETs), and mapping a pixel's temporal sequence onto consecutive word lines (WLs), we enable direct temporal pattern detection within NAND strings. Each NAND string serves as a dedicated reference for a single pixel, while different blocks store patterns for distinct pixels, allowing large-scale spatial-temporal pattern recognition via simple direct bit-line (BL) sensing, a well-established operation in vertical NAND storage. We experimentally validate our approach at both the cell and array levels, demonstrating that vertical NAND-based detector achieves more than six orders of magnitude improvement in energy efficiency and more than three orders of magnitude reduction in latency compared to conventional CPU-based methods. These findings establish vertical NAND storage as a scalable and energy-efficient solution for next-generation neuromorphic vision processing.

==> 06_statement.tex <==

\section*{\textcolor{sared}{Acknowledgments}}

\subsection*{Author contributions}
X.Y., T.K., and K.N. proposed and supervised the project. F.M., M.L., R.O., N.L., S.D., and Z.Z. performed the experimental verification of the proposed design. Q.H., C.L., Z.Y., J.C., Z.S., Y.S. and C.Z. conducted SPICE simulations and verification. M.I. performed system level benchmarking. All authors contributed to write up of the
manuscript.

\subsection*{Competing interests}
\label{sec:conflict}
The authors declare no conflicts of interest.

\subsection*{Data and materials availability}
\label{sec:data}

The data that support the plots within this paper and other findings of this study are
available from the corresponding author on reasonable request.

% \section*{Code availability}
% \label{sec:data}

% Custom code used in this study is available from the corresponding authors upon reasonable request.

==> coverletter.tex <==


\newpage

\noindent
Dear Editors and Reviewers,

\noindent
Please find the enclosed manuscript entitled \textbf{"An In-Situ Spatial-Temporal Sequence Detector for Neuromorphic Vision Sensor Empowered by High-Density Vertical NAND Storage"}, which we submit for consideration in \textit{Nature Communications}. Our work addresses the critical research gap of efficient hardware for processing data streams from neuromorphic vision sensors. For the first time, we demonstrate that large-capacity vertical NAND storage, without requiring modifications to the array structure, can perform in-situ spatial-temporal sequence detection in a massively parallel fashion directly within storage, offering superior energy efficiency and excellent latency.

\noindent
\textbf{Key contributions of our work include:}

\begin{itemize}
    \item \textbf{Innovative Cell Encoding with Multi-Level Cell (MLC) Transistors:} \\ 
    We introduce a novel cell structure composed of two consecutive transistors in series with MLC states to map four pixel states at a given time step: dark-to-bright change, bright-to-dark change, no change, and a "don't care" masking state. By encoding the stored threshold voltage (V\textsubscript{TH}) states and applying input-dependent read voltages, the cell becomes conductive only when the stored information matches the incoming pixel state.

    \item \textbf{String Operations for Temporal Sequence Detection:} \\ 
    We propose a unique mapping method that enables a NAND string to process temporal sequences. By leveraging the serial connection of cells, each representing one time step, a NAND string can inherently detect the temporal sequence of a pixel.

    \item \textbf{Novel Spatial-Temporal Mapping Scheme:} \\ 
    We develop a new mapping approach that allows an entire vertical NAND array to perform spatial-temporal sequence detection in a massively parallel fashion. In our scheme, all reference template sequences for one pixel are stored within a block, while different pixels are mapped to separate blocks. The vertical NAND's massive number of bit lines enables simultaneous searching of all reference template sequences for each pixel.
\end{itemize}

\noindent
Through these innovative designs, commercial vertical NAND storage can be directly employed for spatial-temporal sequence detection, addressing the longstanding need for efficient hardware to process data streams from neuromorphic vision sensors. We firmly believe our work offers a significant contribution to the field.

\noindent
We sincerely appreciate your consideration of our manuscript and look forward to engaging with the reviewers' insightful feedback.


\noindent
Sincerely, \\
Kai Ni
